Assistive Large Language Model Agents for Socially-Aware Negotiation Dialogues

We develop assistive agents based on Large Language Models (LLMs) that aid interlocutors in business negotiations. Specifically, we simulate business negotiations by letting two LLM-based agents engage in role play. A third LLM acts as a remediator agent to rewrite utterances violating norms for improving negotiation outcomes. We introduce a simple tuning-free and label-free In-Context Learning (ICL) method to identify high-quality ICL exemplars for the remediator, where we propose a novel select criteria, called value impact, to measure the quality of the negotiation outcomes. We provide rich empirical evidence to demonstrate its effectiveness in negotiations across three different negotiation topics. We have released our source code and the generated dataset at: https://github.com/tk1363704/SADAS.

==> latex/section/back-mcts.tex <==

A core challenge in the architecture of our ICL-based LLM Assistant is memory management, where to ensure that the most suitable pieces of the conversation memory that are involving with norm violations can be retrieved and synthesized when needed.
We employ a \textbf{memory module}, which maintains a comprehensive \textbf{experience pool} of the agents' past conversations.
The Experience Pool contains a list of memory objects, where each object contains a bargaining dialogue, the violation sentence, and the remediation sentence.

% Each memory object is indexed with the dialogue as the key.
% When retrieving the most relevant memory objects, the input query is the current conversation where a norm violation occurred.
Through this query retrieval process, it is possible to obtain historical dialogues in the memory that can most describe the current query.
Our architecture implements a retrieval function that takes the agent’s current conversation as input and returns a subset of the memory objects to pass on to the language model as the ICL examples.

There are many possible implementations of a retrieval function, depending on what is important for the agent to consider when deciding how to act.
In our context, we focus on one main metric, i.e., informativeness, to produce effective results.
Informativeness assigns a higher score to memory objects that can help describe the task and thus yield negotiation benefits.
% If the query, for example, is that a seller is saying something that would impair the relationship with the buyer when bargaining with the house price, memory objects about the seller and buyer talking about income should have low relevance, whereas memory objects about the house price negotiation should have high relevance.
% In our implementation, we generate an embedding vector of the violation sentence of each memory and maintain the embedding by a vector store.
% Then, we calculate relevance as the cosine similarity between the memory’s embedding vector and the query memory’s embedding vector.
The memories with top scores that fit within the language model’s context window are viewed as the ICL examples and included in the prompt for remediation generation.

Selecting the optimal combination of ICL examples in $S_a$ is an NP-hard combinatorial optimization problem.
Because the order of ICL examples also impacts the model's performance, traversing and evaluating all possible permutations and combinations of ICL examples is inherently infeasible.
We propose a filtering method based on information gain, which can find an approximation of the optimal ICL example set with near-linear computational complexity.
The method consists of two steps: first, identify individuals with the highest informativeness values from $S_a$; second, combine these individuals into an ICL example set and iteratively find the set with the highest informativeness value through random replacement until convergence.
Below, we provide a detailed explanation of these two steps.

\paragraph{Individual Examples Filtering.}
In the first stage, we aim to find those individual examples that have the highest informativeness.
We propose InfoValue (Informativeness Value) to measure the individual in-context informativeness of one example $e = \{x, y\}$ for ICL based on the final negotiation outcome as:
\begin{equation}
I(e, D) = \frac{\sum_{e' \in D} c(e, e')}{|D_v|}
\label{informativeness}
\end{equation}
\begin{equation}
c(e, e') = o(y'|x,y,x') - o(y'|x')
\label{difference}
\end{equation}
In this work, $e' = \{x', y'\}$ signifies initiating a dialogue between the buyer and seller until the first occurrence of a norm violation. 
The conversation up to this norm violation is denoted as $x'$, and the remediation generated in response to the norm violation is denoted as $y'$.
After rewriting $x'$ with $y'$, the conversation continues until it concludes (we control the dialogue generation to prevent any further norm violations).
The negotiation outcome for this conversation includes whether a deal was reached, the transaction price, and whether the business relationship and trust between the negotiating parties deepened, marked as $o(y'|x')$.
The difference between $o(y'|x')$ (obtained using zero-shot prompt-based LLM for $(e, e')$) and $o(y'|x, y, x')$ (obtained using $e = \{x, y\}$ as an ICL example) represents the informativeness gain.
A higher value suggests greater informativeness gain from $e = \{x, y\}$ for the task of $e' = \{x', y'\}$, indicating more significant assistance provided by $e = \{x, y\}$ for this specific task.
Here, if either $o(y'|x')$ or $o(y'|x, y, x')$ leads to the final breakdown of the transaction, it is not considered a `valid comparison'.
Therefore, in equation~\ref{informativeness}, $|D_v|$ refer to the number of valid comparisons that occur in the $D$.

As mentioned earlier, we aim to identify individuals in $S_a$ with the highest InfoValue.
However, the large number of instances in $S_a$ results in lengthy computation times.
To address this, we randomly sample $N$ examples from $S_a$ with a uniform distribution (where $N$ is an order of magnitude smaller than $|S_a|$), forming the candidate set $C$ for ICL examples. Simultaneously, we employ a simulation method to generate a controlled training set $D$ (ensuring only one norm violation occurs in the conversation).
Therefore, we achieve filtering examples with high in-context informativeness value in the complexity of $O(N * |D|)$, where $|D|$ is the size of training set. 

\paragraph{ICL Example Set Search.} As known from previous research, the combination of ICL examples often provides more assistance to the model in understanding the task and brings about information gain compared to a single ICL example.
Moreover, the arrangement order of ICL examples also influences the final inference results.
Therefore, after completing the first step, we need to find an approximately optimal ICL example set that can most effectively help the model solve the current task.
As shown in the algorithm, we first sort the elements in $C$ in descending order based on their InfoValue and take the top-k elements to form the initial ICL example set $S_{ICL}$.
Then, from the remaining elements in $C$, we select the element $c$ with the highest InfoValue, replace it with a randomly selected element from $S_{ICL}$, and obtain $S'_{ICL}$.
Referring to the equation~\ref{informativeness} and equation~\ref{difference}, we have the similar equations:
\begin{equation}
I(e, e', D) = \frac{\sum_{x' \in D} c(e, e', x')}{|D_v|}
\label{informativeness_set}
\end{equation}
\begin{equation}
c(e, e', x') = o(y'|e, x') - o(y'|e', x')
\label{difference_set}
\end{equation}
where $e = S_{ICL}$, $e' = S'_{ICL}$, $|D_v|$ refer to the number of valid comparisons, and $o(y'|e, x')$ denotes the negotiation outcome when the ICL examples in $e$ are used for instructing the model to generate remediation $y'$ to rectify the norm violation $x'$.
It is worth noting that we generate a different training dataset $D$ than what is used in the equation~\ref{informativeness}.

Afterward, we get the value $I(e, e', D)$.
If $I(e, e', D)$ is greater than $0$, we continue to replace a random element in $S'_{ICL}$ with the highest-ranked element from the remaining elements in $C$.
If, in $M$ consecutive replacements, $I(e, e', D)$ is always less than or equal to 0, it is considered as convergence.
At this point, no further replacements are made, and instead, in order to measure the influence of the ordering, the elements obtained in $S'_{ICL}$ are randomly shuffled to get $S''_{ICL}$, and the comparison of $I(S'_{ICL}, S''_{ICL}, D)$ is continued.
Again, when $I(S'_{ICL}, S''_{ICL}, D)$ is less than or equal to 0 for $M$ consecutive times, it is considered converged, and no further reordering is performed.
In the end, the obtained $S''_{ICL}$ is considered as an approximately optimal ICL example set for use in the inference of the test dataset. 








